Poncelet Plectra: Harmonious Curves in Cosine Space

It has been shown that the family of Poncelet N-gons in the confocal pair (elliptic billiard) conserves the sum of cosines of its internal angles. Curiously, this quantity is equal to the sum of cosines conserved by its affine image where the caustic is a circle. We show that furthermore, (i) when N=3, the cosine triples of both families sweep the same planar curve: an equilateral cubic resembling a plectrum (guitar pick). We also show that (ii) the family of triangles excentral to the confocal family conserves the same product of cosines as the one conserved by its affine image inscribed in a circle; and that (iii) cosine triples of both families sweep the same spherical curve. When the triple of log-cosines is considered, this curve becomes a planar, plectrum-shaped curve, rounder than the one swept by its parent confocal family.

==> 120_app_symbols.tex <==
\begin{table}[H]
%\small
\begin{tabular}{|c|l|}
\hline
symbol & meaning \\
\hline
$\E,\E_c$ & outer and inner ellipses \\
$\theta,\theta_i$ & confocal and excentral angles \\
$a,b$ & outer ellipse semi-axes' lengths \\
$a_c,b_c$ & inner ellipse semi-axes' lengths \\
$s,s'$ & \makecell[lt]{affine constants taking confocals (resp.\ excentrals)\\to the incircle (resp.\ circumcirlce) family}\\
\hline
\end{tabular}
\caption{Symbols of used herein.}
\label{tab:symbols}
\end{table}

==> 130_app_jacobi.tex <==

%\label{sec:02-confocal-jacobi-param}
The notation adopted below takes after \cite{armitage2006}. 

\begin{definition}
The incomplete elliptic integral of the first kind $K(\varphi,k)$ is given by:
\begin{equation}
K(\varphi,k)=\int_0^{\varphi}\frac{d\theta}{\sqrt{1-k^2 \sin^2\theta}}
\label{eqn:02-ellipticK}
\end{equation}
%\end{definition}
\index{elliptic integral}
%\begin{definition}
The complete elliptic integral of the first kind $K(k)$ is simply $K(\pi/2,k)$.
\end{definition}

\begin{definition}
The elliptic sine $\text{sn}$, cosine $\text{cn}$, and delta-amplitude $\text{dn}$ are given by:
\begin{align*}
\text{sn}(u,k)&=\sin\varphi\\
\text{cn}(u,k)&=\cos\varphi\\
\text{dn}(u,k)&=\sqrt{1- k^2\sin^2\varphi}\\
\end{align*}
where $\varphi=\text{am}(u,k)$ is known as the amplitude, i.e., the upper-limit in the integral in \cref{eqn:02-ellipticK} such that $K(\varphi,k)=u$.
\end{definition}
For in-depth coverage of these functions see \cite{armitage2006}. Note: Wolfram Mathematica (resp. Maple) expects $m=k^2$ (resp. $k$) as the second parameter to elliptic functions.



==> 999_refcheck.tex <==

\usepackage{refcheck}
% make refcheck work w cref
% https://tex.stackexchange.com/questions/87610/making-refcheck-work-with-cleveref
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

==> _not_used/130_proof_thm_scale.tex <==
Without loss of generality we can restrict to the case with an isosceles triangle, where one vertex of the triangle lies on the endpoint of the major-semi-axis of $\E$ and the other two vertices lie parallel to the minor-axis (see \cref{fig:isosceles}).
For the sum of cosines in this configuration thus follows
\[\sum_{i=1}^{3}\cos(\theta_i)=\cos(\pi-2\theta)+2\cos(\theta)\]

Using trigonometric identities on can relate the cosine sum to the slope 
%
\[m=\tan(\theta)=\frac{a+r}{r\sqrt{\frac{a+r}{a-r}}}=\frac{\sqrt{a^2-r^2}}{r}\]
%
as
%
\[\cos(\pi-2\theta)+2\cos(\theta)=\frac{m^2-1}{m^2+1}+\frac{2}{\sqrt{1+m^2}} \]
%
Under the unique affine transformation only the $x-$coordinates get transformed corresponding to $m\rightarrow \sqrt{\lambda}\cdot m$, i.e. the sum of cosines in the transformed version reads
%
\begin{equation} \label{eq:sum_cos_transformed}
\cos(\pi-2\theta_{\lambda})+2\cos(\theta_{\lambda})=\frac{\lambda m^2-1}{\lambda m^2+1}+\frac{2}{\sqrt{1+\lambda m^2}}
\end{equation}
%
For the sum of cosines \eqref{eq:sum_cos_transformed} to be invariant \eqref{eq:sum_cos} under the transformation we thus obtain after some simple algebraic manipulations the defining equation
%
\begin{center}
\begin{align*}
 1+\frac{2r\cdot (a-r)}{a^2}=\frac{\lambda(a^2-r^2)-r^2}{\lambda(a^2-r^2)+r^2}+\frac{2r}{\sqrt{\lambda(a^2-r^2)+r^2}}\\
 \leftrightarrow \left(1+\frac{2r\cdot (a-r)}{a^2}\right)\cdot \left(\lambda(a^2-r^2)+r^2\right)=\lambda(a^2-r^2)-r^2+2r\sqrt{\lambda(a^2-r^2)+r^2}\\
 \leftrightarrow \frac{\lambda \cdot(a-r)\cdot (a^2-r^2)}{a^2}+\frac{r^2a+r\cdot(a^2-r^2)}{a^2}=\sqrt{\lambda(a^2-r^2)+r^2}
\end{align*}
\end{center}


By squaring both sides the above equation becomes a quadratic equation in $\lambda$ which can be solved using the quadratic formula. The only positive solution is given by

\begin{equation}
\lambda = \frac{(2a-r)\cdot r^3}{(a^2-r^2)\cdot (a-r)^2}
\end{equation}

Since the affine transformation maps the incircle case to ellipse case and it is commonly known that the sum of cosines is invariant for the 1d-family the transformation is valid for the entire family.




\begin{figure}[htb]
\centering
\begin{tikzpicture}[scale=1.7]
\draw[green!60!black, thick] (3,0) arc (0:360:3 and 1.5) node[below] at (3.2,0) {$a$};
\node[green!60!black,left] at (0,1.7) {$\frac{ar}{a-r}$};
\draw[dashed,green!60!black, thick] (-3,0)--(3,0);
\draw[dashed,green!60!black, thick] (0,-1.5)--(0,1.5);
\draw[blue, thick] (0,0) circle (1) node[below] at (1.2,0) {$r$};
\draw[orange, thick] (-3,0)--(1,-1.41)--(1,1.41)--(-3,0);

\fill[orange] (-3,0) circle (0.03) node[left] {$P_1(-a|0)$};
\fill[orange] (1,-1.41) circle (0.03) node[below] {$P_2(r|-r\sqrt{\frac{a+r}{a-r}})$};
\fill[orange] (1,1.41) circle (0.03) node[above] {$P_3(r|r\sqrt{\frac{a+r}{a-r}})$};

\draw (-2,0) arc (0:20:1);
\draw (-2,0) arc (0:-20:1);
\draw[white,ultra thick] (-2.8,0)--(-2.1,0);
\node[right] at (-2.8,0) {$\pi -2\theta$};

\draw (1,1) arc (270:200:0.41) node[above] at (0.85,1.1) {$\theta$};
\draw (1,-1) arc (90:160:0.41) node[below] at (0.85,-1.1) {$\theta$};

\end{tikzpicture}
\caption{Isosceles triangle configuration with symmetry axis being the ellipse major-axis. \label{fig:isosceles}}
\end{figure}







==> _not_used/140_proof_thm_scale2.tex <==
The proof mimicis the proof already performed for the incircle case. Consider therefore without loss of generality the configuration shown in \cref{fig:circumcircle_proof}. The product of cosines thus an be expressed in terms of the tangens as
\[\prod_{i=1}^3 \cos \theta_i=\frac{1-\tan^2 \beta}{(1+\tan^2 \alpha)\cdot (1+\tan^2 \beta)}\]

Under the affine transformation \cref{eq:lambda-matrix} the product of cosines thus transforms as

\[\prod_{i=1}^3 \cos \theta_i'=\frac{1-\frac{1}{\lambda}\cdot\tan^2 \beta}{(1+\lambda \cdot\tan^2 \alpha)\cdot (1+\frac{1}{\lambda}\cdot \tan^2 \beta)}\]

For the invariance the two products have to be equal. A straight forward calculation using
\[\tan^2\beta=\frac{R-a}{R+a}\;\;\;\mbox{and}\;\;\;\tan^2\alpha=\frac{R+a}{R-a}\]

which can be derived using simple trigonometric considerations, then yields the stated result

\[\lambda=\frac{(R-a)^2+R\cdot (R-a)}{a\cdot (a+R)}\]


\begin{figure}[htb]
\centering
\begin{tikzpicture}[scale=1.3,yscale=2]
\draw[green!60!black, thick] (3,0) arc (0:360:3 and 1.5) node[right] at (3.05,0) {$R$};
\node[green!60!black,above] at (0,1.55) {$R$};
\draw[dashed,green!60!black, thick] (-3,0)--(3,0);
\draw[dashed,green!60!black, thick] (0,-1.5)--(0,1.5);
\draw[blue, thick] (0,0) circle (1) node[below] at (1.2,0) {$a$};
\draw[orange, thick] (-3,0)--(1,-1.41)--(1,1.41)--(-3,0);

\fill[orange] (-3,0) circle (0.03) node[left] {$P_1(-R|0)$};
\fill[orange] (1,-1.41) circle (0.03) node[below] at (1,-1.46) {$P_2(a|-\sqrt{R^2-a^2})$};
\fill[orange] (1,1.41) circle (0.03) node[above] at (1.3,1.46) {$P_3(a|\sqrt{R^2-a^2})$};

\draw (-2,0) arc (0:20:1);
\draw (-2,0) arc (0:-20:1);
%\draw[white,ultra thick] (-2.8,0)--(-2.1,0);
\node[right,fill=white] at (-2.7,0) {$2\beta$};

\draw (1,1) arc (270:200:0.41) node[above] at (0.85,1.1) {$\alpha$};
\draw (1,-1) arc (90:160:0.41) node[below] at (0.85,-1.1) {$\alpha$};

\end{tikzpicture}
\caption{Isosceles triangle configuration with symmetry axis being the ellipse major-axis. \label{fig:circumcircle_proof}}
\end{figure}
